CASOG: Conservative Actor-critic with SmOoth Gradient for Skill Learning in Robot-Assisted Intervention

Robot-assisted intervention has shown reduced radiation exposure to physicians and improved precision in clinical trials. However, existing vascular robotic systems follow master-slave control mode and entirely rely on manual commands. This paper proposes a novel offline reinforcement learning algorithm, Conservative Actor-critic with SmOoth Gradient (CASOG), to learn manipulation skills from human demonstrations on vascular robotic systems. The proposed algorithm conservatively estimates Q-function and smooths gradients of convolution layers to deal with distribution shift and overfitting issues. Furthermore, to focus on complex manipulations, transitions with larger temporal-difference error are sampled with higher probability. Comparative experiments in a pre-clinical environment demonstrate that CASOG can deliver guidewire to the target at a success rate of 94.00\% and mean backward steps of 14.07, performing closer to humans and better than prior offline reinforcement learning methods. These results indicate that the proposed algorithm is promising to improve the autonomy of vascular robotic systems.

==> sections/environment.tex <==
\section{Environment}
\label{section: environment}

\subsection{Environment setting}
\label{subsection: environment}

\begin{figure}[t!]
    \centering
    \subfigure[]{
    \includegraphics[width=0.5\linewidth]{figs/environment.pdf}
    \label{subfig: environment}
    }
    \subfigure[]{
    \includegraphics[width=0.2\linewidth]{figs/closeup.png}
    \label{subfig: vessel model}
    }
    \subfigure[]{
    \includegraphics[width=0.2\linewidth]{figs/target.png}
    \label{subfig: target path}
    }
    \caption{The pre-clinical environment. (a) The whole pre-clinical environment. (b) Closeup of the vascular model and guidewire. (c) The outset, target, and correct path.}
    % }
    \label{fig: environment}
\end{figure}

The preclinical environment is similar to that in our previous work\cite{DSAC-AE}, consisting of a vascular robotic system, a guidewire, a catheter and a vascular model as shown in Fig. \ref{subfig: environment}.
The closeup of the vascular model and guidewire is shown in Fig. \ref{subfig: vessel model}.
A Terumo RF*GA35153M guidewire is actuated by the vascular robotic system (here-inafter referred to as robot) with two degrees of freedom (translation and rotation) to a target position in a 3D-printed vascular model.
For details of the robot, we refer readers to \cite{Zhao2021DesignAP}.
The size of the vascular model is 15$\times$15$\times$1 cm.
The vessels are about 3$\sim$5 mm thick in the model.
Volunteers controls the robot with a gamepad for offline data collection.
Details of offline data collection is shown in Section \ref{subsection: offline data collection}.

\subsection{Problem definition}
\label{subsection: problem definition}
To apply RL, Partially Observable Markov Decision Process (POMDP) is used to define the guidewire delivery task.
A POMDP is described by the tuple $\langle\mathcal{S}, \mathcal{O}, \mathcal{A}, P, R, \gamma\rangle$, where $\mathcal{S}, \mathcal{O}, \mathcal{A}$ represent state space, action space, and observation space respectively.
$P: \mathcal{S}\times\mathcal{A}\times\mathcal{S}\mapsto\left[0,1\right]$ is the transition probability,
and $R:\mathcal{S}\times\mathcal{A}\mapsto\mathbb{R}$ is the reward function. $\gamma$ is the discount factor.
Trajectories start in initial states where the distal tip of the guidewire is 10$\sim$15 pixels from the outset and the guidewire is rotated randomly.
At time step $t$, the robot receives an observation $o_t$ and follows policy $\pi$ to choose an action $a_t$.
\begin{figure}
    \centering
    \subfigure[]{
    \includegraphics[width=0.2\linewidth]{figs/vessel.jpg}
    \label{subfig: preprocessed vessel}
    }
    \subfigure[]{
    \includegraphics[width=0.2\linewidth]{figs/gw.jpg}
    \label{subfig: preprocessed guidewire}
    }
    \caption{Prepossessed images as observations in POMDP. (a): The vessel. (b): The guidewire}
    \label{fig: prepossessed observation}
\end{figure}
Then the state of environment $s_t$ changes to $s_{t+1}$ according to the transition probability $P(s_{t+1}|s_t, a_t)$, and the robot gets a reward $r_t=R(s_t, a_t)$ and a new observation $o_{t+1}$.
The maximum time step is 200.
The goal is to find the optimal policy that maximizes discounted cumulative reward $\sum_{t}\mathbb{E}_{o_t,a_t}(\gamma^t r_t)$.
Q-funtion $Q(a,o)$is the expected long-term cumulative reward with initial observation $o$ and initial action $a$, which be regarded as the evaluation of action $a$ under observation $o$.
For offline RL, only offline data can be used for policy optimization.
The details of the POMDP are as follows.

\textbf{Observation:}
The observation is the vertical view of the vascular model with size of 140$\times$140. 
The observation is prepossessed into binary images of the vessel and the guidewire as shown in Figure \ref{fig: prepossessed observation}.

\textbf{Action:}
Actions are speed commands in translation and rotation freedom.
The action space consists of ten discrete actions.
% Ten discrete actions are designed. 
There are two sub-actions in the translation freedom, which are forward and backward with the same speed, and five sub-actions in the rotation freedom, including static, two-speed counterclockwise and clockwise rotation.
The interval between actions is 0.5 seconds.

\textbf{Reward:}
The reward is designed for efficacy and safety, consisting of the dense sub-reward and the safe sub-reward.
The dense sub-reward that encourages the guidewire to to approach the target along the correct path. 
The correct path is the shortest path from the outset to the target as shown in Figure \ref{subfig: target path}, which is automatically generated by the Dijkstra algorithm.
When the guidewire keeps on the correct path, the robot will get a reward that is equal to the decrease in distance to the target. 
The distance of each point to the target is calculated by the Dijkstra algorithm simultaneously with the correct path.
The robot will get a penalty of size 20 if the guidewire deviates from the correct path and goes into a wrong vessel branch, and a bonus of size 20 if the guidewire leaves the wrong vessel branch and goes back to the correct path.
The robot will receive another penalty of size 50 if the guidewire exits the vascular model.
The safe sub-reward. The robot will get a large penalty of size 20 if the contact force between the robot and the guidewire exceeds a safe threshold.
The contact force is represented by the motor current.

